Differentially Private Video Activity Recognition

In recent years, differential privacy has seen significant advancements in image classification; however, its application to video activity recognition remains under-explored. This paper addresses the challenges of applying differential privacy to video activity recognition, which primarily stem from: (1) a discrepancy between the desired privacy level for entire videos and the nature of input data processed by contemporary video architectures, which are typically short, segmented clips; and (2) the complexity and sheer size of video datasets relative to those in image classification, which render traditional differential privacy methods inadequate. To tackle these issues, we propose Multi-Clip DP-SGD, a novel framework for enforcing video-level differential privacy through clip-based classification models. This method samples multiple clips from each video, averages their gradients, and applies gradient clipping in DP-SGD without incurring additional privacy loss. Moreover, we incorporate a parameter-efficient transfer learning strategy to make the model scalable for large-scale video datasets. Through extensive evaluations on the UCF-101 and HMDB-51 datasets, our approach exhibits impressive performance, achieving 81% accuracy with a privacy budget of epsilon=5 on UCF-101, marking a 76% improvement compared to a direct application of DP-SGD. Furthermore, we demonstrate that our transfer learning strategy is versatile and can enhance differentially private image classification across an array of datasets including CheXpert, ImageNet, CIFAR-10, and CIFAR-100.

==> tables/hyperparameters.tex <==
\begin{table*}[htbp]

\centering
\caption{\tb{Hyperparameters.}
}
\label{tab:hyper}
\begin{tabular}{llclccc}
\toprule
Dataset
& Architecture
& Batch size
& \#Epochs
& Scheme
& Learning rate
\\
\midrule

\parbox[t]{20mm}{\multirow{2}{*}{CIFAR-10}}
& \parbox[t]{20mm}{\multirow{2}{*}{ViT-S/16-224}}
& \parbox[t]{10mm}{\multirow{2}{*}{1,024}}
& \parbox[t]{10mm}{\multirow{2}{*}{10}}
&Full fine-tune & 3e-4 \\

&&&& Adapter & 1e-3 \\


\midrule
\parbox[t]{20mm}{\multirow{5}{*}{CIFAR-100}}
& \parbox[t]{20mm}{\multirow{5}{*}{ViT-S/16-224}}
& \parbox[t]{10mm}{\multirow{5}{*}{1,024}}
& \parbox[t]{10mm}{\multirow{5}{*}{50}}
& From scratch & 3e-3 \\

&&&& Full fine-tune & 3e-4 \\

&&&& Linear probe & 1e-3 \\

&&&& Sparse fine-tune & 1e-3 \\

&&&& Adapter & 1e-3 \\


\midrule
\parbox[t]{20mm}{\multirow{5}{*}{CIFAR-100}}
& \parbox[t]{20mm}{\multirow{5}{*}{ConvNeXt-T}}
& \parbox[t]{10mm}{\multirow{5}{*}{1,024}}
& \parbox[t]{10mm}{\multirow{5}{*}{50}}
& From scratch & 5e-3 \\

&&&& Full fine-tune & 7e-4 \\

&&&& Linear probe & 1e-3 \\

&&&& Sparse fine-tune & 1e-3 \\

&&&& Adapter & 1e-3 \\


\midrule
\parbox[t]{20mm}{\multirow{4}{*}{CIFAR-100}}
& \parbox[t]{20mm}{\multirow{4}{*}{ResNet-50-GN}}
& \parbox[t]{10mm}{\multirow{4}{*}{1,024}}
& \parbox[t]{10mm}{\multirow{4}{*}{50}}
& From scratch & 3e-3 \\

&&&& Full fine-tune & 7e-4 \\

&&&& Linear probe & 5e-3 \\

&&&& Sparse fine-tune & 1e-3 \\



\midrule
\parbox[t]{20mm}{\multirow{4}{*}{ImageNet}}
& \parbox[t]{20mm}{\multirow{4}{*}{ViT-S/16-224}}
& \parbox[t]{10mm}{\multirow{4}{*}{1,024}}
& \parbox[t]{10mm}{\multirow{4}{*}{90}}
&Full fine-tune & 1e-4 \\

&&&& Linear probe & 5e-4 \\

&&&& Sparse fine-tune & 5e-4 \\

&&&& Adapter & 5e-4 \\

\midrule

\parbox[t]{20mm}{\multirow{3}{*}{ImageNet}}
& \parbox[t]{20mm}{\multirow{3}{*}{ViT-S/16-224}}
& \parbox[t]{10mm}{\multirow{3}{*}{65,536}}
& \parbox[t]{10mm}{\multirow{3}{*}{70}}
&Full fine-tune & 3e-4 \\


&&&& Sparse fine-tune & 5e-3 \\

&&&& Adapter & 5e-3 \\



\midrule
\parbox[t]{20mm}{\multirow{3}{*}{ImageNet}}
& \parbox[t]{20mm}{\multirow{3}{*}{ViT-B/16-224}}
& \parbox[t]{10mm}{\multirow{3}{*}{65,536}}
& \parbox[t]{10mm}{\multirow{3}{*}{70}}
&Full fine-tune & 1e-4 \\

&&&& Sparse fine-tune & 5e-3 \\

&&&& Linear probe & 5e-3 \\

\midrule
\parbox[t]{20mm}{\multirow{4}{*}{CheXpert}}
& \parbox[t]{20mm}{\multirow{4}{*}{ViT-B/16-224}}
& \parbox[t]{10mm}{\multirow{4}{*}{256}}
& \parbox[t]{10mm}{\multirow{4}{*}{10}}
& From scratch & 1e-4 \\

&&&&Full fine-tune & 3e-4 \\

&&&& Sparse fine-tune & 1e-3 \\


&&&& Adapter & 1e-3 \\

\midrule
\parbox[t]{20mm}{\multirow{4}{*}{CheXpert}}
& \parbox[t]{20mm}{\multirow{4}{*}{ConvNeXt-T}}
& \parbox[t]{10mm}{\multirow{4}{*}{256}}
& \parbox[t]{10mm}{\multirow{4}{*}{10}}
& From scratch & 3e-3 \\

&&&&Full fine-tune & 3e-4 \\

&&&& Sparse fine-tune & 1e-3 \\


&&&& Adapter & 3e-3 \\


\midrule
\parbox[t]{20mm}{\multirow{3}{*}{UCF-101}}
& \parbox[t]{20mm}{\multirow{3}{*}{MViT-B/16×4}}
& \parbox[t]{10mm}{\multirow{3}{*}{16}}
& \parbox[t]{10mm}{\multirow{3}{*}{10}}
&Full fine-tune & 3e-4 \\

&&&& Sparse fine-tune & 3e-4 \\

&&&& Adapter & 3e-4 \\


\midrule
\parbox[t]{20mm}{\multirow{3}{*}{HMDB-51}}
& \parbox[t]{20mm}{\multirow{3}{*}{MViT-B/16×4}}
& \parbox[t]{10mm}{\multirow{3}{*}{16}}
& \parbox[t]{10mm}{\multirow{3}{*}{10}}
&Full fine-tune & 7e-4 \\

&&&& Sparse fine-tune & 4e-3 \\

&&&& Adapter & 9e-4 \\
\bottomrule
\end{tabular}
\label{tab:hyper}
\end{table*}


